Trans-Encoder: Unsupervised sentence-pair modelling through self- and mutual-distillations

In NLP, a large volume of tasks involve pairwise comparison between two sequences (e.g. sentence similarity and paraphrase identification). Predominantly, two formulations are used for sentence-pair tasks: bi-encoders and cross-encoders. Bi-encoders produce fixed-dimensional sentence representations and are computationally efficient, however, they usually underperform cross-encoders. Cross-encoders can leverage their attention heads to exploit inter-sentence interactions for better performance but they require task fine-tuning and are computationally more expensive. In this paper, we present a completely unsupervised sentence representation model termed as Trans-Encoder that combines the two learning paradigms into an iterative joint framework to simultaneously learn enhanced bi- and cross-encoders. Specifically, on top of a pre-trained Language Model (PLM), we start with converting it to an unsupervised bi-encoder, and then alternate between the bi- and cross-encoder task formulations. In each alternation, one task formulation will produce pseudo-labels which are used as learning signals for the other task formulation. We then propose an extension to conduct such self-distillation approach on multiple PLMs in parallel and use the average of their pseudo-labels for mutual-distillation. Trans-Encoder creates, to the best of our knowledge, the first completely unsupervised cross-encoder and also a state-of-the-art unsupervised bi-encoder for sentence similarity. Both the bi-encoder and cross-encoder formulations of Trans-Encoder outperform recently proposed state-of-the-art unsupervised sentence encoders such as Mirror-BERT and SimCSE by up to 5% on the sentence similarity benchmarks.

==> backup.tex <==
\begin{table}[!t] %[!htbp]
\setlength{\tabcolsep}{3.6pt}
%\renewcommand{\arraystretch}{0.8}
\centering
%\scriptsize
\begin{tabular}{lccccccccccc}
\cmidrule[1.5pt]{1-10}
dataset$\rightarrow$  & STS12 & STS13 & STS14 & STS15 & STS16 & STS-B & SICK-R & avg.\\
\cmidrule[1.5pt]{1-10}
Sentence-BERT & 70.97 & 76.53 & 73.19 & 79.09 & 74.30 & 77.03 & 72.91 & 74.89 \\
\cmidrule[1.0pt]{1-10}
\textit{self-distillation results} \\
\cmidrule[1.0pt]{1-10}
SimCSE-BERT-base$\star$ & 68.64 & 82.39 & 74.30 & 80.69 & 78.71 & 76.54 & 72.22 & 76.21 \\
%\hdashline
%\rowcolor{blue!10}
+ \modelname (bi) & 73.33 & 84.28 & 75.90 & 82.77 & 80.22 & 79.92 & 73.97 & 78.63 \\
%\rowcolor{blue!10}
+ \modelname (cross) & 74.22 & 84.72 & 75.87 & 82.51 & 79.83 & 80.07 & 74.52 & 78.82 \\
\cmidrule[0.5pt]{1-10}
SimCSE-RoBERTa-base$\star$ & 68.34 & 80.96 & 73.13 & 80.86 & 80.61 & 80.20 & \textbf{68.62} & 76.10 \\
%\hdashline
%\rowcolor{blue!10}
+ \modelname (bi) &  71.22 & 83.56 & 75.93 & 82.99 & 81.98 & 82.15 & 67.85 & 77.95 \\
%\rowcolor{blue!10}
+ \modelname (cross) & 72.60 & 83.65 & 76.42 & 83.75 & 82.61 & 83.11 & 69.94 & 78.87 \\
\cmidrule[.5pt]{1-10}
SimCSE-BERT-large$\star$  & 71.30 & 84.32 & 76.32 & 84.28 & 79.78 & 79.04 & 73.88 & 78.42  \\
%\hdashline
%\rowcolor{blue!10}
+ \modelname (bi) &  73.98 & 85.15 & 77.10 & 84.52 & 80.49 & 82.22 & 74.19 & 79.66 \\
+ \modelname (cross) &  72.76 & 85.03 & 76.46 & 83.86 & 80.45 & 82.10 & 75.38 & 79.43 \\
\cmidrule[.5pt]{1-10}
SimCSE-RoBERTa-large$\star$ & 71.40 & 84.60 & 75.94 & 84.36 & 82.22 & 82.67 & 71.23 & 78.92 \\
%\hdashline
%\rowcolor{blue!10}
+ \modelname (bi) & 76.73 & 86.91 & 79.49 & 87.74 & 84.53 & 86.04 &  \\
+ \modelname (cross) &  77.34 & 87.36 & 80.95 & 88.10 & 84.29 & 86.24 \\
\cmidrule[1.0pt]{1-10}
\textit{mutual-distillation results} \\
\cmidrule[1.0pt]{1-10}
self-distil-base post-hoc ensemble &  \\
\hdashline
SimCSE-base (ensemble) & 70.71 & 83.49 & 76.45 & 83.13 & 81.79 & 81.51 & 71.94 & 78.43 \\
+ \modelname-mutual (bi) \\
+ \modelname-mutual (cross) \\
+ \modelname-mutual (ensemble) \\
\cmidrule[.5pt]{1-10}
self-distil-large post-hoc ensemble &  \\
\hdashline
SimCSE-large (ensemble) & 73.22 & 86.03 & 78.15 & 85.95 & 82.83 & 83.05 & 73.86 & 80.66 \\
+ \modelname-mutual (bi) \\
+ \modelname-mutual (cross) \\
+ \modelname-mutual (ensemble) \\
\cmidrule[1.5pt]{1-10}

\end{tabular}
%\vspace{-2mm}
\caption{English STS. $\star$. STS and SICK-R splitted.}
\label{tab:sts}
%\vspace{-1.5mm}
\end{table}


